Privacy Auditing of Large Language Models

Current techniques for privacy auditing of large language models (LLMs) have limited efficacy -- they rely on basic approaches to generate canaries which leads to weak membership inference attacks that in turn give loose lower bounds on the empirical privacy leakage. We develop canaries that are far more effective than those used in prior work under threat models that cover a range of realistic settings. We demonstrate through extensive experiments on multiple families of fine-tuned LLMs that our approach sets a new standard for detection of privacy leakage. For measuring the memorization rate of non-privately trained LLMs, our designed canaries surpass prior approaches. For example, on the Qwen2.5-0.5B model, our designed canaries achieve $49.6\%$ TPR at $1\%$ FPR, vastly surpassing the prior approach's $4.2\%$ TPR at $1\%$ FPR. Our method can be used to provide a privacy audit of $\varepsilon \approx 1$ for a model trained with theoretical $\varepsilon$ of 4. To the best of our knowledge, this is the first time that a privacy audit of LLM training has achieved nontrivial auditing success in the setting where the attacker cannot train shadow models, insert gradient canaries, or access the model at every iteration.

==> icml_version/dp_background.tex <==
\section{Auditing Differentially Private Language Models}
\label{sec:audit}

\subsection{Background}
We provide a concise overview of differential privacy (DP), private machine learning, and methods to audit the privacy assurances claimed under DP.

\paragraph{Differential Privacy}\label{ssec:dp}

Differential privacy (DP) is widely regarded as the gold standard for ensuring algorithmic privacy \cite{dwork2006calibrating}.
\begin{definition}[$(\varepsilon,\delta)-$ Differential Privacy (DP)] An algorithm $\mathcal{M}$ is considered to be \adp if for any set of events $S\subseteq \text{Range}(\mathcal{M})$ and all neighboring datasets $D, D' \in \mathcal{D}^n$ (where $\mathcal{D}$ represents the set of all possible data points) differing in one element, the following holds:

\begin{equation}
    \Pr[\mathcal{M}(D)\in S] \leq e^{\varepsilon} \Pr[\mathcal{M}(D')\in S] + \delta
\end{equation}
\end{definition}
Informally, within the realm of machine learning, if a training algorithm $\mathcal{M}$ satisfies \adp, then an adversary's ability to determine whether $\mathcal{M}$ was applied to $D$ or $D'$ is limited by $e^{\varepsilon}$, with $\delta$ representing the probability that this upper bound does not hold.

\paragraph{Differentially Private Machine Learning}

Stochastic gradient descent (SGD) can be made differentially private through two modifications: clipping individual gradients to a maximum Euclidean norm of $C$ and adding random noise to the average of a batch of gradients; this method is known as DP-SGD.
Intuitively, clipping restricts the individual impact any sample can have on the model parameters $\theta$, while adding random noise obscures the contributions of any single example.
In practice, the DP-SGD update rule is as follows: let $B$ represent a batch of examples sampled independently from a dataset $D$, each with probability $q$, $\ell$ a loss function, and $\eta$ a learning rate, then
%
\begin{equation}
    \label{eqn:dpsgd}
    \theta \gets \theta - \eta \left(\mathcal{N}(0, \sigma^2I) + %\frac{1}{|B|}
    \sum_{z \in B}  \text{clip}_{C}\left(\nabla_{\theta}\ell(\theta, z)\right)\right)
\end{equation}
where $\text{clip}_C(v)$ projects $v$ onto the $\ell_2$ ball of
radius $C$ with
\[\text{clip}_{C}(v) = v \cdot \min\left\{1, \frac{C}{\|v\|_2}\right.\]

\paragraph{Auditing DP-SGD}

Any differentially private algorithm $\mathcal{M}$ limits an adversary's ability to infer whether $\mathcal{M}$ was trained with $D$ or $D'$.
\citet{kairouz2015composition} show that if $\mathcal{M}$ is \adp, it defines a \emph{privacy region} (a bound on an attacker's TPR and FPR) given by
%
\begin{equation}
\begin{split}
   \hspace{-8pt}\mathcal{R}(\epsilon, \delta) = \{(\alpha, \beta) \mid\ &\alpha + e^{\epsilon}\beta \geq 1-\delta \land
   e^{\epsilon} \alpha + \beta \geq 1-\delta\ \land \\
   & \alpha + e^{\epsilon}\beta \leq e^{\epsilon}+\delta \land
    e^{\epsilon}\alpha + \beta \leq e^{\epsilon}+\delta \}\hspace{-2pt}
\end{split}\label{eqn:eps_region}
\end{equation}

In other words, an \adp algorithm implies a valid region for the type I ($\alpha$) and type II ($\beta$) errors of any test.

The objective of a privacy \emph{audit} is to design a hypothesis test that distinguishes $D$ from $D'$ while minimizing $\alpha$ and $\beta$. Then, we can compute the privacy budget $\epsilon$, for any fixed value of $\delta$.
In practice, for many interesting differentially private algorithms including DP-SGD, one cannot compute the minimum possible values of $\alpha$ and $\beta$ in closed form, and so empirical estimates are necessary.
This is achieved by designing a \emph{distinguisher} that predicts if mechanism $\mathcal{M}$ operated on $D$ or $D'$. 

A recent privacy auditing method that we use in this paper is~\citet{steinke2023privacy} which can provide an audit without needing to train multiple models. However, they are not able to provide a nontrivial result when training on real data in the black-box setting (where the canaries exist in the input space and the attacker observes the loss of the model), and do not provide audits for language models (only computer vision).

\paragraph{Summary of DP Background}
DP-SGD provides a mathematical proof that gives an upper bound on the privacy parameter. A privacy audit is a procedure that provides a lower bound on the privacy parameter. Privacy audits can be used to ascertain the correctness of DP-SGD training and estimate the tightness of analysis. Many privacy auditing methods have been proposed, but no privacy auditing method has been able to provide a nontrivial lower bound of an LLM trained with a realistic DP guarantee~(\(\varepsilon<10\) on real data in the black-box setting in a single run.

% OLD
% \section{Auditing Differentially Private Language Models}
% \label{sec:audit}

% \subsection{Background}
% We provide a concise overview of differential privacy (DP), private machine learning, and methods to audit the privacy assurances claimed under DP.

% \paragraph{Differential Privacy}\label{ssec:dp}

% Differential privacy (DP) is widely regarded as the gold standard for ensuring algorithmic privacy \cite{dwork2006calibrating}.
% \begin{definition}[$(\varepsilon,\delta)-$ Differential Privacy (DP)] An algorithm $\mathcal{M}$ is considered to be \adp if for any set of events $S\subseteq \text{Range}(\mathcal{M})$ and all neighboring datasets $D, D' \in \mathcal{D}^n$ (where $\mathcal{D}$ represents the set of all possible data points) differing in one element, the following holds:

% \begin{equation}
%     \Pr[\mathcal{M}(D)\in S] \leq e^{\varepsilon} \Pr[\mathcal{M}(D')\in S] + \delta
% \end{equation}
% \end{definition}
% Informally, within the realm of machine learning, if a training algorithm $\mathcal{M}$ satisfies \adp, then an adversary's ability to determine whether $\mathcal{M}$ was applied to $D$ or $D'$ is limited by $e^{\varepsilon}$, with $\delta$ representing the probability that this upper bound does not hold.

% \paragraph{Differentially Private Machine Learning}

% Stochastic gradient descent (SGD) can be made differentially private through two modifications: clipping individual gradients to a maximum Euclidean norm of $C$ and adding random noise to the average of a batch of gradients; this method is known as DP-SGD.
% Intuitively, clipping restricts the individual impact any sample can have on the model parameters $\theta$, while adding random noise obscures the contributions of any single example.
% In practice, the DP-SGD update rule is as follows: let $B$ represent a batch of examples sampled independently from a dataset $D$, each with probability $q$, $\ell$ a loss function, and $\eta$ a learning rate, then
% %
% \begin{equation}
%     \label{eqn:dpsgd}
%     \theta \gets \theta - \eta \left(\mathcal{N}(0, \sigma^2I) + %\frac{1}{|B|}
%     \sum_{z \in B}  \text{clip}_{C}\left(\nabla_{\theta}\ell(\theta, z)\right)\right)
% \end{equation}
% where $\text{clip}_C(v)$ projects $v$ onto the $\ell_2$ ball of
% radius $C$ with
% \[\text{clip}_{C}(v) = v \cdot \min\left\{1, \frac{C}{\|v\|_2}\right.\]

% \paragraph{Auditing DP-SGD}

% Any differentially private algorithm $\mathcal{M}$ limits an adversary's ability to infer whether $\mathcal{M}$ was trained with $D$ or $D'$.
% \citet{kairouz2015composition} show that if $\mathcal{M}$ is \adp, it defines a \emph{privacy region} (a bound on an attacker's TPR and FPR) given by
% %
% \begin{equation}
% \begin{split}
%    \hspace{-8pt}\mathcal{R}(\epsilon, \delta) = \{(\alpha, \beta) \mid\ &\alpha + e^{\epsilon}\beta \geq 1-\delta \land
%    e^{\epsilon} \alpha + \beta \geq 1-\delta\ \land \\
%    & \alpha + e^{\epsilon}\beta \leq e^{\epsilon}+\delta \land
%     e^{\epsilon}\alpha + \beta \leq e^{\epsilon}+\delta \}\hspace{-2pt}
% \end{split}\label{eqn:eps_region}
% \end{equation}

% In other words, an \adp algorithm implies a valid region for the type I ($\alpha$) and type II ($\beta$) errors of any test.

% The objective of a privacy \emph{audit} is to design a hypothesis test that distinguishes $D$ from $D'$ while minimizing $\alpha$ and $\beta$. Then, we can compute the privacy budget $\epsilon$, for any fixed value of $\delta$.
% In practice, for many interesting differentially private algorithms including DP-SGD, one cannot compute the minimum possible values of $\alpha$ and $\beta$ in closed form, and so empirical estimates are necessary.
% This is achieved by designing a \emph{distinguisher} that predicts if mechanism $\mathcal{M}$ operated on $D$ or $D'$. 

% A recent privacy auditing method that we use in this paper is~\citet{steinke2023privacy} which can provide an audit without needing to train multiple models. However, they are not able to provide a nontrivial result when training on real data in the black-box setting (where the canaries exist in the input space and the attacker observes the loss of the model), and do not provide audits for language models (only computer vision).

% \paragraph{Summary of DP Background}
% DP-SGD provides a mathematical proof that gives an upper bound on the privacy parameter. A privacy audit is a procedure that provides a lower bound on the privacy parameter. Privacy audits can be used to ascertain the correctness of DP-SGD training and estimate the tightness of analysis. Many privacy auditing methods have been proposed, but no privacy auditing method has been able to provide a nontrivial lower bound of an LLM trained with a realistic DP guarantee~(\(\varepsilon<10\) on real data in the black-box setting in a single run.
% A \emph{privatized gradient} refers to the gradient after clipping, averaging, and adding noise.
% To achieve \adp, $\sigma$ is typically on the order of $\Omega(q\sqrt{T\log(\frac{1}{\delta})}\varepsilon^{-1})$~\cite{abadi2016deep}, where $T$ is the number of gradient descent iterations, though tighter bounds for a given $\sigma$ have been discovered~\cite{mironov2017renyi, dong2019gaussian, koskela2020computing}.
%
% Each DP-SGD iteration satisfies a particular \adp guarantee through the subsampled Gaussian Mechanism~\cite{abadi2016deep}—a combination of data subsampling and Gaussian noise addition. Since DP is resistant to post-processing, this guarantee can be composed over multiple updates to achieve a final \adp guarantee.



==> icml_version/rebuttal_experiment_results.tex <==
\begin{table}[ht]
    \caption{We compare the audited \(\varepsilon\) when training gpt2 with full finetuning (FFT) and LoRA on PersonaChat. Auditing results are similar; at a \(99\%\) CI, the new token canary gives us an audited \(\varepsilon\) of \(0.84\) under FFT and \(0.89\) under LoRA.}
    \resizebox{\textwidth}{!}{%
    \begin{tabular}{c|c|cccccc}
    \toprule
        %special token
        & & new & bigram & unigram & rare & random \\
    \midrule
    \multirow{2}{*}{FFT}     & audit 95\%  &$1.27$  &$0.72$ &$0.42$ &$0.52$ &$0.31$\\ 
    & audit 99\% &$0.84$ &$0.54$ &$0.26$ &$0.34$ &$0.15$\\
    \midrule
    \multirow{2}{*}{LoRA} & audit 95\% & $1.15$ & $0.43$ & $0.17$ & $0.13$ & $0.58$ \\ 
                          & audit 99\% & $0.89$ & $0.26$ & $0.0$  & $0.0$  & $0.30$ \\
                          & PPL & \(23.93\) & \(23.17\) & \(23.15\) & \(24.44\) & \(23.14\)
    \bottomrule
    \end{tabular}
    }
    \label{tab:lora_vs_fft}
\end{table}

\begin{table}[ht]
    \caption{We report the audited value of \(\varepsilon\) across two confidence intervals for different models, all with the new token canary, on PersonaChat, with FFT.}
    \resizebox{\textwidth}{!}{%
    \begin{tabular}{c|ccccc}
    \toprule
        %special token
        & & Pythia-160M & Pythia-140M & gpt2 & gpt2-large & qwen2.5-0.5B \\
    \midrule
    audit 95\%  & \(0.40\) & \(0.67\) & \(1.27\) & \(1.28\) & \(0.96\) \\
    audit 99\% & \(0.25\) & \(0.46\) & \(0.84\) & \(1.08\) & \(0.86\) \\
    % PPL & \(86.99\) & \(21.19\) & & \(14.18\) & \(14.44\) \\
    \bottomrule
    \end{tabular}
    }
    \label{tab:model_comparison}
\end{table}

\begin{table}[ht]
    \caption{We compare the audited value of \(\varepsilon\) when training GPT2 with FFT on PersonaChat and the E2E dataset, for different canary strategies. Auditing results are similar; at a \(99\%\) CI, the new token canary gives us an audited \(\varepsilon\) of \(0.84\) when training on PersonaChat and an audited \(\varepsilon\) of \(0.82\) when training on E2E.}
    \resizebox{\textwidth}{!}{%
    \begin{tabular}{c|c|cccccc}
    \toprule
        %special token
        & & new & bigram & unigram & rare & random \\
    \midrule
    \multirow{2}{*}{PersonaChat}     & audit 95\%  &$1.27$  &$0.72$ &$0.42$ &$0.52$ &$0.31$\\ 
    & audit 99\% &$0.84$ &$0.54$ &$0.26$ &$0.34$ &$0.15$\\
    \midrule
    \multirow{2}{*}{E2E} & audit 95\% & $1.15$ & $0.13$ & $0.03$ & $0.05$ & $0.30$ \\ 
                          & audit 99\% & $0.82$ & $0.0$ & $0.0$  & $0.0$  & $0.10$ \\
                          % & PPL & \(4.45\) & \(4.34\) & \(4.33\) & \(4.52\) & \(4.33\)
    \bottomrule
    \end{tabular}
    }
    \label{tab:lora_vs_fft}
\end{table}

==> icml_version/threat_model.tex <==
\section{Motivation \& Threat Model}

Our research aims to enhance the efficiency of empirical privacy estimation. This improvement enables an examination of the discrepancy between theoretical and practical privacy limits. Additionally, auditing techniques can be employed to verify the accuracy of a differential privacy (DP) implementation. The reliability of our empirical privacy assessments hinges on the specific threat model we employ and the assumptions made about the adversary. ~\citet{nasr2021adversary} outline various threat models and scenarios for auditing machine learning systems protected by differential privacy. We also explore multiple threat models, recognizing the inevitable compromise between the strength of the audit (with a potent adversary) and the audit's applicability to real-world machine learning scenarios (where the assumptions required for a strong adversary might not be realistic). We prioritize three threat models in descending order of attack potency.

\textbf{White-box access with gradient canaries:} This model aligns closely with the threat model presumed by DP and the theoretical analysis of DP-SGD. Here, the adversary has access to the privatized gradient and model parameters at every update step and can select any gradient for each update~\citep{balle2022reconstructing}, termed a canary gradient. This gradient is then incorporated into the update with a certain probability q. This scenario mirrors an adversary who can access all training aspects except the randomness in noise addition and batch selection (i.e., knowing when z was used in training, where \(D'=D\bigcup {z}\).

\textbf{White-box access with input-space canaries:} The previous model assumes the adversary can choose any gradient to be sampled into a batch of updates, which might be impractical. Our second threat model removes this assumption, granting adversaries access to intermediate updates but limiting them to selecting any training sample (from which gradients are computed) rather than choosing a gradient directly. We refer to this training sample chosen for each update as the canary sample. This model is particularly suited to federated learning scenarios, where an adversary can access model updates but may not be able to insert arbitrary gradients into the training pipeline.

\textbf{Gray-box: only has access to final outputs, but has the power to modify model embedding by adding new added tokens.}

\textbf{Black-box access:}  most restrictive rare tokens/no added tokens. no access to gradients, cannot modify model architecture [black-box].  This is one of the most restrictive threat models for conducting audits, where an adversary can only insert a training example at the start of training and observe the model post-training. The adversary cannot see or influence intermediate model updates. Although this is the most limited view from an adversarial standpoint, it is arguably the most realistic in practice. We emphasize that this threat model differs from the typical setting analyzed in DP, which assumes intermediate model updates are visible to the adversary. We include it in our study to assess how progressively limiting adversarial access to model updates and gradients impacts the precision of our lower bound for $\epsilon$.

==> macros.tex <==
Tca\usepackage{listings}
\lstset{escapeinside={<@}{@>}}
\usepackage[scaled=0.85]{beramono}            % load a nice TT font
\lstset{basicstyle=\ttfamily, language=sh, keywords={}, deletekeywords={for,return}}    % set defaults for any listing

\definecolor{color-blind-cyan}{HTML}{56B4E9}
\definecolor{color-blind-orange}{HTML}{E69F00}
\definecolor{color-blind-green}{HTML}{029E73}

\newcommand\cc[1]{{#1}}  % Chris

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% THEOREMS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\theoremstyle{plain}
\newtheorem{theorem}{Theorem}[section]
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{corollary}[theorem]{Corollary}
\theoremstyle{definition}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{assumption}[theorem]{Assumption}
\theoremstyle{remark}
\newtheorem{remark}[theorem]{Remark}

\newcommand{\theoremref}[1]{Theorem~\ref{#1}}
\newcommand{\sectionref}[1]{Sect.~\ref{#1}}
\newcommand{\definitionref}[1]{Definition~\ref{#1}}
\newcommand{\defref}[1]{Definition~\ref{#1}}
\newcommand{\propref}[1]{Proposition~\ref{#1}}
\newcommand{\stepref}[1]{Step~\ref{#1}}
\newcommand{\figureref}[1]{Fig.~\ref{#1}}
\newcommand{\lemmaref}[1]{Lemma~\ref{#1}}
\newcommand{\claimref}[1]{Claim~\ref{#1}}
\newcommand{\remarkref}[1]{Remark~\ref{#1}}
\newcommand{\corollaryref}[1]{Corollary~\ref{#1}}
\newcommand{\inequalityref}[1]{Inequality~\ref{#1}}
\newcommand{\constructionref}[1]{Construction~\ref{#1}}
\newcommand{\itemref}[1]{Item~\ref{#1}}
\newcommand{\propertyref}[1]{Property~\ref{#1}}
\newcommand{\protocolref}[1]{Protocol~\ref{#1}}
\newcommand{\algorithmref}[1]{Algorithm~\ref{#1}}
\newcommand{\appendixref}[1]{Appendix~\ref{#1}} 

\newcommand{\fix}{\marginpar{FIX}}
\newcommand{\new}{\marginpar{NEW}}

\DeclareMathOperator*{\argmin}{\arg\!\min}
\DeclareMathOperator*{\argmax}{\arg\!\max}

\newcommand{\E}{\mathbb{E}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\eps}{\varepsilon}
\newcommand{\D}{\mathcal{D}}
\newcommand{\norm}[1]{\left\lVert#1\right\rVert}
\newcommand{\N}{\mathcal{N}}
%\newcommand{\I}{\mathcal{I}}
\newcommand{\M}{\mathcal{M}}
\newcommand{\Ind}{\mathds{1}}
\newcommand{\g}{\nabla}
\newcommand{\iden}{\bm{1}}
\newcommand{\inner}[2]{\left\langle #1, #2 \right\rangle}

\newcommand{\EXP}{\text{Exp}}
\newcommand{\LLM}{ \textbf{LLM} }
\newcommand{\GPT}{ \textbf{GPT} }

\newcommand{\cX}{\mathcal{X}}
\newcommand{\cY}{\mathcal{Y}}
\newcommand{\cZ}{\mathcal{Z}}
\newcommand{\MS}{\mathrm{MultiSets}}

\newcommand{\PromptAtt}{\textsc{Prompt}\textsubscript{Att}}
\newcommand{\PromptSec}{\textsc{Prompt}\textsubscript{Sec}}

\newif\ifshowcomments

\showcommentstrue 
%\showcommentsfalse

\ifshowcomments
\newcommand {\yaoqing}[1]{{\color{cyan}\sf{[Yaoqing: #1]}}}
\newcommand {\prateek}[1]{{\color{red}\sf{[Prateek: #1]}}}
\else
\newcommand {\yaoqing}[1]{{\color{cyan}\sf{}}}
\newcommand {\prateek}[1]{{\color{red}\sf{}}}
\fi

% \newcommand {\yaoqing}[1]{}

\newcommand{\adp}[0]{$(\varepsilon,\delta)$-DP\xspace}
\newcommand{\pdp}[0]{$\varepsilon$-DP\xspace}

